Task Success Prediction for Open-Vocabulary Manipulation Based on Multi-Level Aligned Representations

In this study, we consider the problem of predicting task success for open-vocabulary manipulation by a manipulator, based on instruction sentences and egocentric images before and after manipulation. Conventional approaches, including multimodal large language models (MLLMs), often fail to appropriately understand detailed characteristics of objects and/or subtle changes in the position of objects. We propose Contrastive $\lambda$-Repformer, which predicts task success for table-top manipulation tasks by aligning images with instruction sentences. Our method integrates the following three key types of features into a multi-level aligned representation: features that preserve local image information; features aligned with natural language; and features structured through natural language. This allows the model to focus on important changes by looking at the differences in the representation between two images. We evaluate Contrastive $\lambda$-Repformer on a dataset based on a large-scale standard dataset, the RT-1 dataset, and on a physical robot platform. The results show that our approach outperformed existing approaches including MLLMs. Our best model achieved an improvement of 8.66 points in accuracy compared to the representative MLLM-based model.

==> sections/sup/qualitative_failure.tex <==
\section{Failure Examples of Contrastive $\lambda$-Repformer}
\input{figures/qualitative-failure}

Fig.~\ref{fig:qualitative-failure} shows failed cases of the proposed method. The left and right images represent the scene before and after manipulation, respectively.
Fig.~\ref{fig:qualitative-failure} (i) shows an example with the instruction of ``open middle drawer.'' The ground truth label for this example was success, because the robot opened the middle drawer. Nonetheless, our method predicted that the robot failed in carrying out the instruction. This error can be explained by the fact that most of the middle drawer lies outside the photographed area, making it hard even for humans to deduce correctly.

The instruction for the instance displayed in Fig.~\ref{fig:qualitative-failure} (ii) is ``pick orange from white bowl'' and the ground truth label was failure. This result is most likely because the bottom of the orange is still touching the other oranges. Meanwhile, all the baseline and proposed methods predicted success. This error arises from the ambiguity of the situation, where predictions would likely be divided even among humans.

% HSR
% 110 FN
% move the mug near the spam can

% 103 FP
% move the apple close to the red can

==> sections/sup/quantitative_comparison_few_shot_prompting.tex <==
% the following section is added in rebuttal
\input{figures/few_shot_samples}
\section{Quantitative Comparison Against Foundation Models with Few-Shot Prompting}
\vspace{-2mm}
We compared the performance of Contrastive $\lambda$-Repformer with few-shot prompted foundation model methods using GPT-4V \citep{gpt4v} and Gemini \citep{team2023gemini}.
The models were provided with an instruction-based prompt, three positive and three negative samples from the training split of the SP-RT-1 dataset, along with the sample to be evaluated.
The instruction-based prompt given to GPT-4V was ``Two images, taken from a single viewpoint camera, show the robot executing an instruction. Based on the images and the instruction, please determine whether the robot has successfully completed the task and answer with `true' or `false'.''
The instruction-based prompt given to Gemini was ``These images show the robot executing an instruction. The first image shows the scene before the object manipulation by the robot and the second image shows the scene after. Based on the two images and the instruction, determine whether the robot has successfully completed the task and answer with only `true' or `false'.''
The samples provided to the MLLMs are shown in Fig.~\ref{fig:few_shot_samples} with its instruction. The samples were randomly selected.

\input{tables/fewshot_prompting}

Table~\ref{tab:quantitative_fewshot_prompting} shows additional quantitative results of a comparison between few-shot prompted foundation model methods and Contrastive $\lambda$-Repformer.
As shown in Table~\ref{tab:quantitative_fewshot_prompting}, Contrastive $\lambda$-Repformer outperformed both the few-shot prompted GPT-4V and Gemini methods on the SP-RT-1 dataset, which had accuracies of 72.10\% and 69.20\%, respectively.
In the zero-shot transfer experiment, the Contrastive $\lambda$-Repformer achieved superior performance to the few-shot prompted GPT-4V and Gemini methods, with accuracies of 54\% and 56\%, respectively.


==> tables/fewshot_prompting.tex <==
\begin{wraptable}{r}{0.6\textwidth}
    \centering
    % \vspace{-15mm}
    {%
    % \footnotesize
    \begin{tabular}{lcc}
        \toprule
        Model & \multicolumn{2}{c}{Accuracy [\%]} \\
        & SP-RT-1 & Zero-shot transfer \\
        \midrule
        GPT-4V~\citep{gpt4v} (Few-Shot) & 72.10 & 54 \\
        Gemini~\citep{team2023gemini} (Few-Shot) & 69.20 & 56 \\
        Contrastive $\lambda$-Repformer & \textbf{80.80} & \textbf{60} \\
        \bottomrule \\

    \end{tabular}
    \vspace{-15pt}
    }
    \caption{\small Quantitative results of few-shot prompted foundation model and proposed methods on the SP-RT-1 dataset and the results of the zero-shot transfer experiment. Bold indicates the accuracy with the highest value. }
    \label{tab:quantitative_fewshot_prompting}
\end{wraptable}
